Superpixel Tokenization for Vision Transformers: Preserving Semantic Integrity in Visual Tokens

Transformers, a groundbreaking architecture proposed for Natural Language Processing (NLP), have also achieved remarkable success in Computer Vision. A cornerstone of their success lies in the attention mechanism, which models relationships among tokens. While the tokenization process in NLP inherently ensures that a single token does not contain multiple semantics, the tokenization of Vision Transformer (ViT) utilizes tokens from uniformly partitioned square image patches, which may result in an arbitrary mixing of visual concepts in a token. In this work, we propose to substitute the grid-based tokenization in ViT with superpixel tokenization, which employs superpixels to generate a token that encapsulates a sole visual concept. Unfortunately, the diverse shapes, sizes, and locations of superpixels make integrating superpixels into ViT tokenization rather challenging. Our tokenization pipeline, comprised of pre-aggregate extraction and superpixel-aware aggregation, overcomes the challenges that arise in superpixel tokenization. Extensive experiments demonstrate that our approach, which exhibits strong compatibility with existing frameworks, enhances the accuracy and robustness of ViT on various downstream tasks.

==> figures/dino_attention.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{raw_figures/dino_attentions_4.pdf}
    \caption{\textbf{Self-attention map comparison between DINO-ViT and DINO-\ours.} All maps are visualized by averaging the [CLS] token's self-attention from the final layer across all heads.}
    \label{fig:dino_attention} 
\end{figure}


==> figures/rebut_id.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.6\linewidth]{raw_figures/rebut_class_ident.pdf} 
    \caption{class ident.}
    \vspace{-1em}
    \label{fig:rebut_id} 
\end{figure}


==> figures/rebuttal_fig.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{raw_figures/rebuttal_fig.pdf} 
    \vspace{-2em}
    \caption{\textbf{(Left)} Visualization of Grid vs. Spxl tokenization. \textbf{(Right)} K-means clustering results of SPiT vs. SuiT (Ours).}
    \vspace{-2.5em}
    \label{fig:rebuttal_fig} 
\end{figure}


==> tables/finetuning.tex <==
\begin{table}[t!]
    \centering
    \begin{tabular}{l c c c}
    \toprule
         & Tiny & Small & Base \\
    \midrule\midrule
        Quadformer~\cite{quadformer} & - & 80.8 & 84.4 \\
        MSViT~\cite{msvit} & 75.5 & 82.0 & - \\
        \ours (Fine-tuned) & \textbf{76.1} & \textbf{82.6} & \textbf{84.5} \\
    \midrule
        SPiT~\cite{spit} & - & 75.0 & 80.4 \\
        \ours (Scratch) & \textbf{75.7} & \textbf{80.9} & \textbf{82.1} \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison with existing studies on tokenization.} Experiment above reports the Top-1 accuracy on ImageNet-1K. The numbers for Quadformer-Tiny, MSViT-Base and SPiT-tiny are intentionally left blank, as they are unavailable.}
    \label{tab:finetuning}
\end{table}

==> tables/finetuning_revised.tex <==
\begin{table}[t!]
    \centering
    \begin{tabular}{l c c c}
    \toprule
         & Tiny & Small & Base \\
    \midrule\midrule
        Quadformer~\cite{quadformer} & - & 80.8 & 84.4 \\
        MSViT~\cite{msvit} & 75.5 & 82.0 & - \\
        \ours (Fine-tuned) & \textbf{76.1} & \textbf{82.6} & \textbf{84.5} \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Comparison with existing studies on tokenization.} Experiment above reports the Top-1 accuracy on ImageNet-1K. The numbers for Quadformer-Tiny, MSViT-Base and SPiT-tiny are intentionally left blank, as they are unavailable.}
    \label{tab:finetuning_revised}
\end{table}

==> tables/main_in1k.tex <==
\begin{table}[t!]
    \centering
    \adjustbox{width=\linewidth}{
    \begin{tabular}{c c c c c c}
    \toprule
         Size & Model & \# Params. & GMACs & \# tokens & Top-1 \\
    \midrule\midrule
        \multirow{4}{*}{Tiny} & DeiT & 5.7M & 1.26 & 196 & 72.2\\
        \cmidrule{2-6}
        &\multirow{3}{*}{\shortstack[c]{\ours}} & \multirow{3}{*}{5.5M} & 0.79 & 100 & \underline{72.2} \\
        & & & \underline{1.26} & 171 & 75.3 \\
        & & & 1.44 & \underline{196} & \textbf{75.7} \\
    \midrule
        \multirow{4}{*}{Small} & DeiT & 22.1M & 4.61 & 196 & 79.8\\
        \cmidrule{2-6}
        & \multirow{3}{*}{\shortstack[c]{\ours}} & \multirow{3}{*}{21.7M} & 3.64 & 132 & \underline{79.8} \\
        & & & \underline{4.60} & 172 & 80.5 \\
        & & & 5.20 & \underline{196} & \textbf{80.9} \\
    \midrule
        \multirow{4}{*}{Base} & DeiT & 86.8M & 17.6 & 196 & 81.8 \\
        \cmidrule{2-6}
        & \multirow{3}{*}{\shortstack[c]{\ours}} & \multirow{3}{*}{86.0M} & 16.4 & 160 & \underline{81.8} \\
        & & & \underline{17.6} & 173 & 82.0 \\
        & & & 19.7 & \underline{196} & \textbf{82.1} \\
     \bottomrule
    \end{tabular}}
    \caption{\textbf{Comparison of classification performance on ImageNet-1K against DeiT.} The performance of \ours is reported with varying token counts. Underlined values indicate those that match DeiT's GMACs or token counts.
    }
    \label{tab:in1k}
\end{table}
